SMDP-Based Dynamic Batching for Efficient Inference on GPU-Based Platforms

In up-to-date machine learning (ML) applications on cloud or edge computing platforms, batching is an important technique for providing efficient and economical services at scale. In particular, parallel computing resources on the platforms, such as graphics processing units (GPUs), have higher computational and energy efficiency with larger batch sizes. However, larger batch sizes may also result in longer response time, and thus it requires a judicious design. This paper aims to provide a dynamic batching policy that strikes a balance between efficiency and latency. The GPU-based inference service is modeled as a batch service queue with batch-size dependent processing time. Then, the design of dynamic batching is a continuous-time average-cost problem, and is formulated as a semi-Markov decision process (SMDP) with the objective of minimizing the weighted sum of average response time and average power consumption. The optimal policy is acquired by solving an associated discrete-time Markov decision process (MDP) problem with finite state approximation and "discretization". By introducing an abstract cost to reflect the impact of "tail" states, the space complexity and the time complexity of the procedure can decrease by 63.5% and 98%, respectively. Our results show that the optimal policies potentially possess a control limit structure. Numerical results also show that SMDP-based batching policies can adapt to different traffic intensities and outperform other benchmark policies. Furthermore, the proposed solution has notable flexibility in balancing power consumption and latency.

==> Data/GPU_Performance_Evaluation.tex <==
\section{GPU Performance Evaluation for Machine Learning Inference Tasks}\label{sec:GPU}
To start with, we need to evaluate the GPU performance and acquire the attribute of the service time for machine learning inference tasks.

The calculation performed in inference tasks is predefined, since the dimension of input and the layers in the neural networks are all fixed.
Therefore, no matter what the exact inputs are, the inference task takes the same quantity of multiplication and addition operations, and thus the service time should be considered to be deterministic.
It has been examined in \cite{ali2020batch} that the coefficient of variation (CV) of service time of a specific inference task is always smaller than 0.1, which is near deterministic (CV=0).

In \cite{inoue2021queueing,ali2020batch,shi2022multi}, the authors propose that the inference latency grows linearly with the batch size. We carried out experiments on our GPU server, which is a NVDIA TITAN xp, to profile the relationship between latency and GPU batch size. The statistics are plotted in Fig.~\ref{fig:3dssd},\ref{fig:mobilenet}, which are tested on 3DSSD\cite{yang20203dssd} and MobileNetv2\cite{sandler2018mobilenetv2}, respectively.
In these figures, the latency of each layer is plotted and the throughput is calculated by batch size divided by total latency consumed from input to output layer.


% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{Fig/latency_batchsize_3dssd.pdf}
%     \caption{Latency and throughput of GPU (NVIDIA TITAN xp) regarding batch size on 3DSSD task.}
%     \label{fig:3dssd}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{Fig/latency_batchsize_mobilenetv2.pdf}
%     \caption{Latency and throughput of GPU (NVIDIA TITAN xp) regarding batch size on MobileNetv2 task.}
%     \label{fig:1}
% \end{figure}

\begin{figure}[htbp]
	\centering
	\begin{minipage}{0.49\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{Fig/latency_batchsize_3dssd.pdf}
% 		\caption{GPU (NVIDIA TITAN xp) performance tested on 3DSSD\cite{yang20203dssd} task.}
        \caption{GPU performance tested on 3DSSD\cite{yang20203dssd}.}
		\label{fig:3dssd}%文中引用该图片代号
	\end{minipage}
	%\qquad
	\begin{minipage}{0.49\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{Fig/latency_batchsize_mobilenetv2.pdf}
% 		\caption{GPU (NVIDIA TITAN xp) performance tested on MobileNetv2\cite{sandler2018mobilenetv2} task.}
		\caption{GPU performance tested on MobileNetv2\cite{sandler2018mobilenetv2}.}
		\label{fig:mobilenet}%文中引用该图片代号
	\end{minipage}
\end{figure}

The statistics acquired by us are similar to those in \cite{ali2020batch,inoue2021queueing,NVIDIA}.
We discover that both inference latency and throughput are monotonically increasing with regard to the batch size.
Specifically, the increase of throughput regarding batch size implies that the computational efficiency of GPU gets larger as more tasks are batched together, and also the benefit of batching shows degression law of marginal effect.


The latency is almost linear with batch size, just as the relation discovered by others.
We give the quantitative approximation model of latency by linear regression, and the model of throughput is acquired as well.
We take the statistics of 3DSSD as example, and the regression is shown in Fig.~\ref{fig:fitting}.

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{Fig/curvefitting.jpg}
    \caption{Curve fitting for GPU performance on 3DSSD task.}
    \label{fig:fitting}
\end{figure}

Similarly, the energy consumption is linear to batch size as well according to \cite{inoue2021queueing}, and the curve of energy efficiency regarding batch size is similar to that of throughput.



==> Data/abstract.tex <==
\begin{abstract}
% In the era of artificial intelligence (AI) and internet of things (IoT), machine learning (ML) inference will be widely deployed in ubiquitous devices to take the responsibility of smart sensing, detection, decision, etc.
In the era of artificial intelligence (AI) and internet of things (IoT), machine learning (ML) inference is widely deployed in ubiquitous devices for smart sensing, detection, decision, etc.
Graphics processing units (GPUs) are important computation resources for emerging ML applications because of their excellent performance in parallel computing.
% However, the deployment of GPU is restricted by the considerable monetary cost in both purchasing the hardware and the electric charge when running the device.
% However, powerful GPUs are mostly deployed in cloud or edge servers restricted by the considerable monetary cost in both purchasing the hardware and the electrical charge when running the device.
However, the deployment of GPU is restricted by considerable monetary cost and thus most ML tasks are offloaded from users to GPU-based servers.
% Compared to ML training tasks, the workload of ML inference tasks is usually light, which leads to a huge waste in the traditional GPU renting service mode.
% Compared to ML training tasks, the workload of ML inference tasks is usually light, which makes it inefficient and wasteful for a single user to rent a GPU server.
Compared to ML training tasks, the workload of ML inference tasks is usually light, which makes it inefficient and wasteful to provide GPU renting for a single user.
In the up-to-date serverless computing setting where users only send computation tasks to the platform without considering the hardware, the inference tasks from different users can be batched and processed together so as to improve the efficiency of GPU. 

We adopt the dynamic batching technique and formulate a Markov decision problem to get the optimal batching policy.
Both model-based value iteration algorithm and model-free reinforcement learning algorithm are applied to solve this problem.
It can be observed that the optimal policy has a threshold structure.
Simulation results demonstrate that the optimal batching policy can balance the average queue length and energy consumption compared to other batching policies. 



% Serverless computing is a new pay-per-use cloud service paradigm that automates resource scaling for stateless functions and can potentially facilitate bursty machine learning serving. Batching is critical for latency performance and cost- effectiveness of machine learning inference, but unfortunately it is not supported by existing serverless platforms due to their stateless design. Our experiments show that without batching, machine learning serving cannot reap the benefits of serverless computing. In this paper, we present BATCH, a framework for supporting efficient machine learning serving on serverless platforms. BATCH uses an optimizer to provide inference tail latency guarantees and cost optimization and to enable adaptive batching support. We prototype BATCH atop of AWS Lambda and popular machine learning inference systems. The evaluation verifies the accuracy of the analytic optimizer and demonstrates performance and cost advantages over the state-of-the-art method MArk and the state-of-the-practice tool SageMaker.
\end{abstract}


==> Data/abstract_v1.tex <==
\begin{abstract}
In the era of artificial intelligence (AI) and internet of things (IoT), machine learning (ML) inference widely exists in ubiquitous devices and graphics processing units (GPUs) are important computation resources for ML.
For inference tasks that come in a bursty manner with light workload, it has been found that the batching effect can be further exploited in the up-to-date serverless computing paradigm.
% where users send their tasks to the computing platform without specifying the hardware.
The basic idea is to batch inference tasks from different users together in the serverless platform so as improve the efficiency of GPU. 
A larger batch size leads to higher computation and energy efficiency but probably longer sojourn time. Therefore the batch size should be chosen dynamically and carefully. 
The optimal dynamic batching problem is concluded to a control problem in a batch service queuing system. 
An infinite-horizon average cost problem is formulated as a Markov decision process (MDP) with the objective of minimizing the weighted sum of average AoI and average energy consumption.
Therefore, in this paper formulate a Markov decision problem to get the optimal batching policy.
Both model-based value iteration algorithm and model-free reinforcement learning algorithm are applied to solve this problem.
It can be observed that the optimal policy has a threshold structure.
Simulation results demonstrate that the optimal batching policy can balance the average queue length and energy consumption compared to other batching policies. 



% Serverless computing is a new pay-per-use cloud service paradigm that automates resource scaling for stateless functions and can potentially facilitate bursty machine learning serving. Batching is critical for latency performance and cost- effectiveness of machine learning inference, but unfortunately it is not supported by existing serverless platforms due to their stateless design. Our experiments show that without batching, machine learning serving cannot reap the benefits of serverless computing. In this paper, we present BATCH, a framework for supporting efficient machine learning serving on serverless platforms. BATCH uses an optimizer to provide inference tail latency guarantees and cost optimization and to enable adaptive batching support. We prototype BATCH atop of AWS Lambda and popular machine learning inference systems. The evaluation verifies the accuracy of the analytic optimizer and demonstrates performance and cost advantages over the state-of-the-art method MArk and the state-of-the-practice tool SageMaker.
\end{abstract}


==> Data/algorithm.tex <==
\section{Scheduling with MDP-Based Approach}\label{sec:mdp}
\subsection{Markov Decision Process Formulation}
We consider a continuous time system.
The state in the system is the queue length $s$, $s \in \mathcal{S}=\{0,1,2,\dots,{BF}_{max}\}$, where $\mathcal{S}$ is the state space.
The action $a$ is the batch size, $a \in \mathcal{A}=\{0,1,2,\dots,{B}_{max}\}$, where $\mathcal{A}$ is the state space.
When $a=0$, it means to wait.
By the way, the $a(t)$ should not exceed the current $s(t)$.
The action is made either when the server processes a batch over, or when a task arrives while the server is idle.
We want to acquire a stationary Markovian policy $\pi : \mathcal{S} \rightarrow \mathcal{A}$.

Note that if we consider a system with finite buffer size, then there should be punishment for overflow.
Therefore, we split the state of $s={BF}_{max}$ to two parts, one is ${BF}_{max}^{n}$ with no overflow and another is ${BF}_{max}^{o}$ for the state that should be larger than ${BF}_{max}$ but is set to ${BF}_{max}$ because of overflow.
Then the state space has ${BF}_{max}+1$ dimensions.
${BF}_{max}^{n}$ and ${BF}_{max}^{o}$ stand for the same length of queue, and shows no difference from the view of transition start point.
However, they play an important role in punishing the overflow, i.e. they are different from the view of transition destination.   

And for the case of infinite buffer size, we have to assign a big ${BF}_{max}$ to approximate it, since MDP can only be solved in finite space.

The transition matrix is $P \in \mathbb{R}^{({BF}_{max}+2) \times ({BF}_{max}+2) \times ({B}_{max}+1)}$ and the element $p(s'|s,a)$ is calculated by the Poisson distribution.
% Specifically, we define $\delta$ as $\delta = s'$

\begin{equation}
p(s'|s,a)=
\left\{\begin{array}{l}
\frac{{(\lambda D(a))}^{s'-s+a}}{(s'-s+a)!}e^{- \lambda D(a)}, \;  s'-s+a \geq 0, \;0<a \leq s, \; s',s \in \mathcal{S}, \; a \in \mathcal{A}, \; s' \neq {BF}_{max}^{o}\\
\sum_{i=s'-s+a+1}^{\infty}\frac{{(\lambda D(a))}^{i}}{i!}e^{- \lambda D(a)}, \;  s'-s+a \geq 0, \;0<a \leq s, \; s \in \mathcal{S}, \; a \in \mathcal{A}, \; s' = {BF}_{max}^{o}\\
1, \; s = {BF}_{max} \;or\; {BF}_{max}^{o}, \; a=0, \; s' = {BF}_{max}^{o}\\
1, \; s < {BF}_{max} , \; a=0, \; s' = s+1\\
0, \; \text{otherwise}
\end{array}\right. .
\label{eq12}
\end{equation}

We take (\ref{objective}) as the objective and the corresponding reward matrix is defined as $R \in \mathbb{R}^{({BF}_{max}+2) \times ({BF}_{max}+2) \times ({B}_{max}+1)}$ and the element $R(s'|s,a)$ is:
\begin{equation}
    R(s'|s,a)=
    \left\{\begin{array}{l}
-\text{overflow cost}, \; s' = {BF}_{max}^{o} \\    
-w1*i-w2*E(a), \;  s'-s+a \geq 0, \;a \leq s, \; s',s \in \mathcal{S}, \; a \in \mathcal{A}, \; s' \neq {BF}_{max}^{o}, \; a \neq 0\\   
-w1*i, \;  s'-s+a \geq 0, \; s',s \in \mathcal{S}, \; s' \neq {BF}_{max}^{o}, \; a = 0\\ 
-{BF_{max}}^2, \; \text{otherwise}
\end{array}\right. .
\end{equation}

\subsection{Relative Value Iteration (RVI) for MDP with Average Cost}
Value iteration algorithm is numerically unstable for MDP with average cost\cite{robbins1951stochastic}.
Instead, we use \emph{relative} value iteration\cite{bertsekas2011dynamic} algorithm to solve the problem.
The value function of state $s$ in the $n$th epoch is defined as $J^n(s)$.
In the RVI algorithm, a common bias is deleted from the value function, for example the value of a given state.
Although the relative value function is not the original state value, it does not effect the policy of maximizing the reward.

\begin{algorithm}
\begin{minipage}{1\linewidth}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\caption{Relative Value Iteration Algorithm} 
	\begin{algorithmic}[1]
    	\REQUIRE {$S$: All states; $R(s'|s,a)$: Immediate reward matrix;}
	    \ENSURE {${\pi}_q^{*}$;}
	    \STATE {Initialize $J^0(s)=0$ for all $s \in \mathcal{S}$;}
	    \STATE {Randomly select a beginning state $s$ and another state $s^{*}$;}
	    \FOR {$n:=1$ to $\infty$}
	    \FOR {each $s \in \mathcal{S}$}
	    \STATE {Compute $J^{n+1} (s)=\max_a \{E_{s'\sim p(\cdot|s,a)} [R(s'|s,a)+J^n  (s' )]-J^n  (s^{*} )]\}$;}
	    \ENDFOR
	    \IF {$sp(J^{n+1}-J^n)<\epsilon $}
	    \STATE {break;}
	    \ENDIF
	    \ENDFOR
	    \FOR {each $s \in \mathcal{S}$}
	    \STATE {$a^{*}(s) = \arg \max_a \{E_{s'\sim p(\cdot|s,a)} [R(s'|s,a)+J  (s' )]\}$;}
	    \ENDFOR
	    \STATE {
	    ${\pi}_q^{*} = (a^{*}(s_1), a^{*}(s_2), \dots , a^{*}(s_{|S|}))$;
	    }
    \end{algorithmic}
\end{minipage}
\end{algorithm}

\subsection{Visualization of MDP Solution}
In this part, we demonstrate the policies gained by minimizing the weighted objective (\ref{objective}).

First we start with the objective of minimizing the average queue length, which means $w1=1$, $w2=0$ in (\ref{objective}).
The policies are shown in Fig.~\ref{fig:policy1},\ref{fig:policy2},\ref{fig:policy3}.
We observe that the optimal policy owns a threshold structure: When the queue is shorter than the threshold, the server waits for more tasks to arrive; When the queue is longer than the threshold, the server batches all the current tasks and process.

From top to bottom $\rho$ increases from 0.1 to 0.95, and the policy varies from almost work-conservative policy to near maximum batching policy.
This result is reasonable since when the traffic load is light, the cost of waiting is much larger than the benefit. When the traffic load is heavy, it takes relative short time to wait to form a larger batch.


\begin{figure}[htbp]
	\centering
	\begin{minipage}{0.33\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{Fig/policyview_batch16.jpg}
% 		\caption{GPU (NVIDIA TITAN xp) performance tested on 3DSSD\cite{yang20203dssd} task.}
        \caption{Optimal policy (maximum batch size is 16).}
		\label{fig:policy1}%文中引用该图片代号
	\end{minipage}
	%\qquad
	\begin{minipage}{0.33\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{Fig/viewpolicy_batch28.jpg}
% 		\caption{GPU (NVIDIA TITAN xp) performance tested on MobileNetv2\cite{sandler2018mobilenetv2} task.}
		\caption{Optimal policy (maximum batch size is 28).}
		\label{fig:policy2}%文中引用该图片代号
	\end{minipage}
	\begin{minipage}{0.33\linewidth}
		\centering
		\includegraphics[width=0.99\linewidth]{Fig/viewpolicy_batch36.jpg}
% 		\caption{GPU (NVIDIA TITAN xp) performance tested on MobileNetv2\cite{sandler2018mobilenetv2} task.}
		\caption{Optimal policy(maximum batch size is 36).}
		\label{fig:policy3}%文中引用该图片代号
	\end{minipage}
\end{figure}

As for the objective of maximizing energy efficiency, or minimizing average energy cost, the optimal policy is maximum batching, which means that the server waits until the tasks can be formed in to the largest batch size.
This conclusion holds since the energy consumption is modeled as $E(b)=\hat{A}b+\hat{C}$, and $\sum_{i=1}^{n}E(b_i) \geq E(\sum_{i=1}^{n} b_i)$.

Then we compare the optimal policies in different weight settings, shown in Fig~\ref{fig:weightpolicy}.
The first figure shows the optimal policy when $(w1,w2)=(1,0)$, which is to minimize the average queue length. It shows a threshold structure.
The last figure shows the optimal policy when $(w1,w2)=(1,100)$, and it is already the maximum batching policy.
From top to bottom, the weight $w2$ increases and the optimal policy transits from the original threshold policy to maximum batching policy.
It is found that the optimal policy always has the threshold structure no matter the weight.

\begin{figure}
    \centering
    \includegraphics[width=0.4\linewidth]{Fig/policyview_weightedobj.jpg}
    \caption{Optimal policies in different weight settings.}
    \label{fig:weightpolicy}
\end{figure}

==> Data/algorithm2.tex <==
\section{Scheduling with Reinforcement Learning Approach}\label{sec:rl}

\subsection{Relative Value Iteration (RVI) Q-learning for MDP with Average Cost}
The last section provides the classical relative value iteration algorithm for MDP problem with average cost, which is model-based.
For cases that the transition matrix is not available, we need some model-free algorithms, for example Q-learning.
It's special in our problem that the objectives are long-time average ones, so that normal Q-learning algorithms are numerically unstable\cite{bertsekas2011dynamic} in the setting.

In \cite{gosavi2004reinforcement}, the authors conclude two main reinforcement learning algorithms for MDP with average cost: Relative Value Iteration (RVI) Q-learning and Stochastic Shortest Path (SSP) Q-learning, and provide the convergence analyses of the methods.
In our work, we choose the RVI Q-learning algorithm corresponding to aforementioned RVI algorithm.

Define $Q^{n}(s,a)$ as the Q-function of the state action pair $(s,a)$ in the $n$th epoch.

The RVI Q-learning algorithm is updated according to the following equation:
\begin{equation}
Q^{n+1}(s, a)=Q^{n}(s, a)+\gamma(n)\left[R\left(\xi_{s a}^{n}| i,a \right)+\max _{b} Q^{n}\left(\xi_{s a}^{n}, b\right)-f\left(Q^{n}\right)-Q^{n}(s, a)\right] \quad
s \in \mathcal{S}, \; a,b \in \mathcal{A},    
\label{eq:update}
\end{equation}
where $\xi_{s a}^{n}$ are samples independently generated with the law of $\xi_{s a}^{n}$ being $p(\cdot |s, a)$ for all $n$.
$\gamma(k) \in(0, \infty)$ is the learning rate, e.g. $\gamma(k)=\frac{1}{\sqrt{k+2}}$. $f\left(Q^{n}\right)$ is the bias in relative value, e.g. $f\left(Q^{n}\right)=Q^{n}\left(s^{0}, a^{0}\right)$.


\begin{algorithm}
\begin{minipage}{0.7\linewidth}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\caption{RVI Q-Learning Algorithm} 
	\label{alg5}
	\begin{algorithmic}[1]
    	\REQUIRE {$S$: All states; $R(s'|s,a)$: Immediate reward matrix; ${\epsilon}_0$: exploration probability;}
	    \ENSURE {${\pi}_q^{*}$;}
	    \STATE {Initialize $Q(s,a)=0$ for all $s \in \mathcal{S}$ and $a \in \mathcal{A}$;}
	    \STATE {Randomly select a beginning state $s$;}
	    \FOR {$n:=1$ to $\infty$}
	    \STATE {On the current state $s$, generate a probability $p_0 \sim U(0,1)$;}
	    \IF {$p_0 \leq \frac{1}{\sqrt{t}}\epsilon_0$}
	    \STATE {take a random action $a(s)$ with equal probability;}
	    \ELSE
	    \STATE {$a(s) = \arg \max_{a \in \mathcal{A}} Q(s, a)$;}
	    \ENDIF
	    \STATE {Take action $a(s)$ and observe the reward $R(s'|s,a)$ and next state $\xi_{s,a}$;}
	    \STATE {Update the Q-table values using (\ref{eq:update}); }
	    \STATE{Update $s \leftarrow s'$;}
	    \ENDFOR
	    \FOR {each $s \in \mathcal{S}$}
	    \STATE {$a^{*}(s) = \arg \max_{a \in \mathcal{A}} Q(s, a)$;}
	    \ENDFOR
	    \STATE {
	    ${\pi}_q^{*} = (a^{*}(s_1), a^{*}(s_2), \dots , a^{*}(s_{|S|}))$;
	    }
    \end{algorithmic}
\end{minipage}
\end{algorithm}



\subsection{Visualization of RL-Based Solution}
In Fig~\ref{fig:Qvary}, we exhibit the change of policy with the increase of training iterations.
The corresponding objective is to minimize the queue length.
The maximum batch size is set to 16 and $\rho$ is set to 0.9. 

The last figure shows the optimal policy, which is obtained by relative value iteration algorithm.
From 10,000 to 100 million iterations, the output policy is getting closer to the optimal policy, which validates the effectiveness of the Q-learning method.

\begin{figure}
    \centering
    \includegraphics[width=0.97\linewidth, height=0.4\linewidth]{Fig/Qpolicyvary.jpg}
    \caption{The policies gained by RVI Q-Leaning in different iterations.}
    \label{fig:Qvary}
\end{figure}

==> Data/conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}
In this paper, we studied the problem of dynamic batching for machine learning inference on GPU-based servers.
The problem is modeled as an infinite space semi-Markov decision process (SMDP) with the weighted sum of average response time and average energy consumption as the objective. 
The SMDP is solved with finite state approximation, "discretization" transformation and relative value iteration.
And the computational complexity is largely reduced owning to the introduction of an additional cost.
We take the GoogLeNet inference on TESLA P4 as an example and conduct extensive numerical experiments in various parameter settings. 
The observation is that the optimal policies have a control limit structure, which we will try to prove in future work.
The comparison with other policies has validated the superiority of the SMDP solution.
The latency-energy tradeoff curves also exhibit its advantage in flexibly balancing the performance and cost.
% Compared to other dynamic batching schemes, our policy is derived from theoretical analysis, and it releases the system from the burden of additional complex modules such as online profiling and prediction.
% Compared to other dynamic batching schemes, our policy is derived from theoretical analysis and thus is computable.
Compared to existing dynamic batching schemes, our proposed policies are calculable.
% The policies for different traffic intensities and different weights can be calculated offline and stored in a chart.
The policies for different traffic intensities and weights can be computed offline and stored in a chart.
% For policies that possess a control limit structure, only the value of the control limit needs to be stored for representation.
For policies that possess a control limit structure, only the value of the control limit needs to be stored.
When the platform is running, it only looks up the policy in the chart, given the weights and the traffic intensity assessed online.
As a result, our scheme releases the system from the burden of additional complex modules such as online profiling and prediction.
% and it releases the system from the burden of additional complex modules such as online profiling and prediction.
The limitation is that our method only considers the average objective, instead of hard Service-Level
Objective (SLO) constraints, for which our proposed policy can function as a basic guideline and needs to be modified while running in real time.


==> Data/conclusion2.tex <==
\section{Conclusion}\label{sec:conclusion}
In this paper, we studied the problem of dynamic batching for machine learning inference on GPU-based platforms.
The problem is modeled as an infinite state semi-Markov decision process (SMDP) with the weighted sum of average response time and average power consumption as the objective. 
The SMDP is solved with finite state approximation, ``discretization" transformation and relative value iteration.
And the computational complexity is largely reduced owning to the introduction of an abstract cost.
We take the GoogLeNet inference on TESLA P4 as an example and conduct extensive numerical experiments in various parameter settings. 
The observation is that the optimal policies potentially have a control limit structure.
The comparison with other policies has validated the superiority of the SMDP solution.
The latency-energy tradeoff curves also exhibit its advantage in flexibly balancing the performance and cost.
% Compared to other dynamic batching schemes, our policy is derived from theoretical analysis, and it releases the system from the burden of additional complex modules such as online profiling and prediction.
% Compared to other dynamic batching schemes, our policy is derived from theoretical analysis and thus is computable.
Compared to existing dynamic batching schemes, our proposed solution is theoretically derived, rather than simulation tryouts.
% The policies for different traffic intensities and different weights can be calculated offline and stored in a chart.
% The policies for different traffic intensities and weights can be computed offline and stored in a chart that can be looked up while running online.
The SMDP-based policies for different traffic intensities and weights can be computed offline and stored in a lookup table.
As a result, our scheme releases the system from the burden of extra complex modules such as online profiling and prediction.
% and it releases the system from the burden of additional complex modules such as online profiling and prediction.
The limitation is that our method only considers the average objective, instead of hard Service-Level
Objective (SLO) constraints, for which the proposed solution can function as a basic guideline and needs to be modified while running in real time.


==> Data/introduction2.tex <==
\section{Introduction}
% In the era of artificial intelligence (AI) and internet of things (IoT), machine learning (ML) inference widely exists in ubiquitous devices for smart sensing, signal processing, decision, etc.
% Graphics processing units (GPUs) are important computation resources for emerging ML applications because of their excellent performance in parallel computing.

The last decade has witnessed the rapid growth of machine learning (ML), and graphics processing units (GPUs) play a prominent role in accelerating the training and inference of neural networks due to their advantage in parallel computing\cite{oh2004gpu}. 
% Recently, ML is becoming widely used by ubiquitous devices for applications such as content recommendation\cite{da2020recommendation} and health monitoring\cite{sony2019literature}.
% Recently, ML is becoming widely used by ubiquitous devices for applications such as content recommendation and health monitoring.
% However, few powerful computing resources (e.g., GPUs) are locally deployed due to considerable monetary cost.
% As a result, it sparks a growing demand for ML-as-a-Service (MLaaS) platforms such as Google Cloud Prediction, Amazon ML, and Microsoft Azure ML\cite{GoogleCloud,Amazon,Microsoft}, where trained models are published in the cloud to provide
% inference (prediction) services for massive end-users.
% As a result, it sparks a growing demand for ML-as-a-Service (MLaaS) platforms such as Google Cloud Prediction\cite{GoogleCloud}, where trained models are published in the cloud to provide
% inference (prediction) services for massive end-users.
The wide deployment of ML on various devices sparks a growing demand for ML-as-a-Service (MLaaS) platforms such as Google Cloud Prediction\cite{GoogleCloud}, where trained models are published in the cloud to provide
inference (prediction) services for massive end-users.

% The increasing effectiveness of Machine Learning (ML) and the advent of cloud services is producing rapid growth of Machine Learning as a Service (MLaaS) platforms such as IBM Watson, Google
% Cloud Prediction, Amazon ML, and Microsoft Azure ML [1, 2, 5, 7].
% Clients of these platforms create and train ML models, and publish
% them as web services. End-users and client applications then query
% these trained models with new inputs and the services perform
% inference (prediction) [24]. 
% As a powerful computing resource, GPU shows its advantage in parallel computing. 
% Although ML has been widely placed on ubiquitous devices for applications such as content recommendation\cite{da2020recommendation} and smart sensing\cite{spencer2004smart}, the deployment of GPU is hindered by considerable monetary cost and thus many ML tasks are offloaded from users to GPU-based servers.
% ML-as-a-Service: developers train ML
% models and publish them in the cloud as online services to
% provide low-latency inference at scale
% Although ML has been widely used by ubiquitous devices for applications such as content recommendation\cite{da2020recommendation} and smart sensing\cite{spencer2004smart}, the deployment of GPU is hindered by considerable monetary cost and thus many ML tasks are offloaded from users to GPU-based servers.
% Besides offloading, a growing demand of ML-as-a-Service (MLaaS) has been sparked, where trained models are published in the cloud to provide
% inference services for massive users.
% Since ML has been widely applied in fields such as content recommendation\cite{da2020recommendation} and autonomous driving\cite{grigorescu2020survey}, a growing demand of ML-as-a-Service (MLaaS) has been sparked, where trained models are published in the cloud to provide
% inference services for massive users.
% Since ML is going to be widely used by ubiquitous devices probably without powerful computing resources like GPUs, a growing demand of ML-as-a-Service (MLaaS) has been sparked, where trained models are published in the cloud to provide
% inference services for massive users.



% Since the GPU is expensive, many cloud servers and edge servers provide GPU renting service for users. For the inference serving, the tasks of a user often come in a bursty manner with light workload, which is a huge waste of GPU resources.
% Many cloud and edge servers have provided GPU renting service for users.
An important factor that affects both cost and performance of ML inference serving is batch processing, or \emph{batching}\cite{zhang2019mark,crankshaw2017clipper}.
For GPUs, batching brings about a significant increase in both computational efficiency and energy efficiency\cite{NVIDIA},
i.e., the average processing time (energy consumption) per task decreases with the batch size. 
% Therefore, batching is expected to reduce the cost by fewer invocations and less energy consumption.
% TODO:batching can from a same user/ different users, bursty, especially in serverless platforms;
% Nowadays, a new pay-per-use service paradigm called serverless computing\cite{castro2019rise} (also referred to as Function-as-a-Service (FaaS)) has further promoted the use of batching\cite{ali2020batch}.
% In serverless computing, users only provide the source codes of their functions and call the functions without considering resource allocation, instead of running their own virtual machines (VMs) separately in the common Infrastructure-as-a-Service (IaaS) paradigm\cite{zhang2019mark}.
% In serverless computing, users only provide the source codes of their functions and call the functions without considering resource allocation, instead of running their own virtual machines (VMs) separately\cite{zhang2019mark}.
% In serverless computing, users only provide the source codes of their functions and call the functions without considering resource allocation.
As depicted in Fig.~\ref{fig:batching}, the GPU-based computing platform can bundle the same type of inference requests from possibly different users, and serve them concurrently using the same ML application, for example in the scenario of Function as a Service (FaaS)\cite{castro2019rise}.

% Meanwhile, in the new pay-per-use service paradigm called serverless computing (also referred to as Function-as-a-Service (FaaS)), users only provide the source codes of their functions without considering the resource allocation in the hardware\cite{ali2020batch},
% which can better fit the machine learning inference serving.

% In the recent trend that most computing platforms are equipped with GPUs, another key factor that heavily influences both cost and performance of serverless ML inference serving is \emph{batching}\cite{zhang2019mark,crankshaw2017clipper}.
% which can better fit to the machine learning inference serving.



% Another key factor that heavily influences both cost and performance of serverless ML inference serving is \emph{batching}\cite{zhang2019mark,crankshaw2017clipper}.
% With batching, inference requests from possibly different users can be bundled together and served concurrently by the same ML model (as dipicted in Fig.~\ref{fig:batching}).
% Especially for GPUs, \emph{batching} brings about a significant increase in both computational efficiency and energy efficiency\cite{NVIDIA}.
 

% In the most common server renting paradigm, Infrastructure as a Service (IaaS), users run virtual machines (VMs) with resource management
% in terms of vCPUs, memory, storage, and accelerators (e.g., GPU)\cite{zhang2019mark}.
% However, for the inference serving, the tasks of a user often come in a bursty manner with light workload\cite{gujarati2017swayam,tang2019nanily}, which leads to a huge waste of resources.




% Especially for GPUs, both computational efficiency and energy efficiency significantly increase owing to batch processing\cite{NVIDIA,crankshaw2017clipper,zhang2019mark}. 
Despite the well-known benefits, there are two main challenges in batching:
1) Although batching improves the throughput of GPU, the inference response time is likely to increase because of waiting to form a batch, as well as longer processing time of serving more requests at once\cite{ali2020batch,crankshaw2017clipper}.
2) Static configured batching does not fit realistic scenarios\cite{choi2021lazy}, where it shows poor responsiveness at low load and low throughput at high load\cite{cui20202}. 
To tackle these problems, a dynamic batching scheme is required, to judiciously adjust the batch size to balance the performance and cost.

% On the other hand, an online batching scheme is difficult
% --> dynamic batching with judicious parameterization

\begin{figure}
    \centering    \includegraphics[width=0.64\linewidth]{Figures/batching.eps}
    \caption{Batching of the inference requests from different users on a GPU-based platform.}
    \label{fig:batching}
\end{figure}

% There have been methods of dynamic batching\cite{crankshaw2017clipper,serf,cui20202,choi2021lazy} in maching learning inference systems. 
% In the literature, several dynamic batching schemes have been proposed for machine learning inference systems\cite{crankshaw2017clipper,serf,zhang2019mark,cui20202,choi2021lazy,ali2020batch}, and most of them are designed from a systematic perspective.
% Most of them are designed from a systematic perspective, utilizing profiling and prediction modules to dynamically configure the batch size.
% Meanwhile, only a small amount of researches have made progress in theoretical analysis. 
Recently, several dynamic batching schemes have been proposed for machine learning inference systems\cite{crankshaw2017clipper,serf,zhang2019mark,cui20202,choi2021lazy,ali2020batch,yao2022eais}.
Meanwhile, only a small amount of researches have made progresses in the  performance analysis. 
% SERF\cite{serf} models the inference serving as an M/D/c queue and then estimates request latency, but unfortunately batching is not explicitly considered in the model and even the simplified problem has no closed-form solution.
SERF\cite{serf} models the inference serving as a M/D/c queue, but unfortunately batching is not explicitly considered in the model.
% Another work BATCH\cite{ali2020batch} models the request arrival as a Poisson or MMPP(2) process\cite{lu2013approach} and gets the number of requests that arrive before timeout, based on which it determines the distribution of request latency.
% The limitation in \cite{ali2020batch} is that the cases where requests arrive during processing time are missing from the analysis, leading to an incomplete description of the queuing dynamics. Another work BATCH\cite{ali2020batch} models the request arrival as a Poisson or MMPP(2) process\cite{lu2013approach} and gets the number of requests that arrive before timeout, based on which it determines the distribution of request latency.
Another work BATCH\cite{ali2020batch} models the request arrival as a Poisson or MMPP(2) \footnote{MMPP(2) is a Markov-modulated Poisson
process (MMPP) with two phases\cite{lu2013approach}.} process and gets the number of requests that arrive before timeout.
% The limitation of \cite{ali2020batch} is that the cases where requests arrive during processing time are missing from the analysis.
However, the cases that requests arrive during processing time are missing from the analysis.
The author of \cite{inoue2021queueing} gives a closed-form queuing analysis of dynamic batching under the work-conserving policy, which is not optimal since it eliminates the potential of forming larger batches.
  
% In \cite{inoue2021queueing}, the author gives a closed-form queuing analysis of dynamic batching under the work-conserving policy, which is non-optimal since it eliminates the potential of forming larger batches.
% The limitation is that without considering the complete queuing dynamics, the cases where requests arrive during the serving times are missing from the analysis, leading to inaccurate results. 
% The limitation is that BATCH\cite{ali2020batch} only considers the case that the system is initially vacant with an empty buffer.
% Nevertheless, the cases that requests arrive during the serving times are important to the dynamics of the queuing system as well.


% There have been methods of dynamic batching\cite{ali2020batch,choi2021lazy,crankshaw2017clipper} wherein the number of jobs in a batch, i.e. the \emph{batch size}, can be dynamically adjusted. Another parameter \emph{timeout} is also usually mentioned, which means the maximum waiting time to form a batch. 
% From the theoretical perspective, designing the batching policy is an optimal control problem in batch service queues.
% Although there are abundant researches concerning this topic in operational research, they don't cope with our problem where the processing times are batch-dependent, contradicting the i.i.d. assumption in existing researches.
In fact, dynamic batching decision is an optimal control problem in batch service queues.
Although there are abundant researches concerning this topic in operational research\cite{deb1973optimal,papadaki2002exploiting,fowler2021survey}, they do not cope with our problem because of their essential assumption that the processing time of a batch is \emph{independent} of its
batch size.
In \cite{inoue2022load}, the author models the load-balancing problem in multiple batch service queues with \emph{size-dependent} processing time as a Markov decision process (MDP) and claims it as an open problem.
Actually, optimal batching in one such batch service queue, as the simplest sub-problem of \cite{inoue2022load},  still remains unsolved. 

% To the best of our knowledge, our work is the first to formulate the dynamic batching of the machine learning serving into a semi-Markov Decision Process (SMDP) problem, which reduces the dimension of the state space compared to the discrete-time MDP model\cite{inoue2022load}.
To the best of our knowledge, our work is the first to formulate and optimally solve the dynamic batching of inference requests as a semi-Markov decision process (SMDP).
% Through linear regression on realistic statistics, the inference latency and energy consumption are modeled as deterministic linear functions of the batch size. 
The considered objective is a weighted sum of average response time and average power consumption.
To solve the problem, we provide a procedure composed of finite state approximation, model ``discretization" and relative value iteration.
% Furthermore, we provide a procedure composed of state space truncation, model "discretization" and relative value iteration to solve the optimal dynamic batching policy.
% From numerical results, we can observe the structure of the optimal policies as well as the time-energy trade-off.
% The dimension of the approximate state space and the complexity in iteration algorithms are largely reduced
The demanding problem of state space explosion is tackled by a novel introduction of an abstract cost, which reflects the impact of costs in ``tail" states. 
% Its impact on approximation accuracy and complexity is shown by numerical results.
% From numerical results,
% an important observation is that the optimal policies potentially possess a control limit structure, which is exactly the conclusion in batch service queues with i.i.d. batch processing time\cite{deb1973optimal}.
% From numerical results, we observe that the optimal policies potentially possess a control limit structure, which could further benefit the simplification of the representation and computation. 
From numerical results, we observe that the optimal policies potentially possess a control limit structure, which could inspire the simplification of representation and computation in future researches.  
% By comparison with other benchmark policies, the superiority of the proposed SMDP policy is presented.
Comparisons with other benchmarks demonstrate that: 1) The SMDP-based policies always achieve the best objective in different settings of parameters.
2) When having the same average response time, the SMDP-based policies never consume more energy than any other benchmark policy, and vice versa.  
Moreover, the proposed solution can adapt to different traffic intensities, and it can also flexibly balance the response time and power consumption.
% The approximation accuracy and complexity are also discussed in numerical results.
% And the performance gap between static batching policies and our proposed policies is explicitly shown in the latency-energy figures validates the importance of dynamic batching. 

% The superiority of the computed policy is also shown by comparison with other benchmark policies.

% and the optimal dynamic batching policy is provided by solving the problem.
% The main contributions are summerized as follows:


% GPU dynamic batching has only come into the view of researchers these two years, and not many works have been done about it. In this paper, we will formulate the dynamic batching problem and then design a scheduling policy for the multiuser inference in a GPU server, so as to optimize the performance metric.

% This paper is organized as follows: Section~\ref{sec:related} demonstrates the related works, Section~\ref{sec:GPU} exhibits the performance evaluation of GPU, Section~\ref{sec:system} presents the system model.
% In Section~\ref{sec:mdp}, we provide the MDP formulation and the corresponding algorithm.
% In Section~\ref{sec:rl}, we extend the model-based algorithm to the model-free algorithm, which is a reinforcement learning approach.
% Section~\ref{sec:results} shows simulation results of performance comparison.
% Section~\ref{sec:conclusion} concludes the paper.


==> Data/proposaldata.tex <==
\section{Setting and Objective}
This work is considered in a slotted time setting, and the time slot is denoted as $t \in \{1,2,...,T\}$. 
There are $N$ users in this system, and the task of the $i$-th user comes into the service queue $Q_{i}$ of the server, with $Q_{i}(t)$ representing the length of the $i$-th queue at slot $t$, where $i {\in} \{1,2,...,N\}$. 
Suppose that at most one task is generated by the $i$-th user in a slot, which is $A_{i}(t)\in\{0,1\}$. Let $\lambda_{i}=\mathbbm{E}\{A_{i}(t)\}$, which is the arrival rate. 
We assume that the decision of batching is taken immediately at the start of each slot, and the GPU pulls tasks from the queues, which is carried out in negligible time, and starts the computation. 
The pulled tasks in slot $t$ are $\mathbf{S}(t)\triangleq[S_{1}(t),S_{2}(t),...S_{N}(t)]$, $S_{1}(t)\in\{0,1,2,...Q_{i}(t)+A_{i}(t)\}$. 
Also note that $\sum_{i=1}^{N} S_{i}(t)\leq B_{max}$, where $B_{max}$ is the maximum batch size that cannot be exceeded. 
At each time slot, the size of the batch that the GPU is serving is $b(t)\in\{0,1,2,...B_{max}\}$. When $b(t)=0$, it means that the GPU is idle in the current slot. The dynamics of a queue is formulated as follows:

\begin{equation}
\centering
Q_{i}(t+1)=Q_{i}(t)+A_{i}(t)-S_{i}(t).
\end{equation}

Unlike the scheme of batching at the maximum batch size or at the maximum waiting time, in our problem, the timeout in batching is not confined. Instead, the GPU makes decision to form the batch or wait at every idle slot.

One key issue in our problem is the formulation of the GPU's performance with regard to batch size. Since the inference tasks generated at any slot by any user are homogeneous and can be batched together, each task is considered as a standard unit and the performance of the GPU is determined by its intrinsic attribute along with the batch size. The generic form of the execution time for the GPU to compute a batch of $b$ tasks is $D(b)$, and the throughput is $R(b)\triangleq b/D(b)$. To the best of our knowledge, none has ever given 
an exact functional form of the delay or throughput regarding batch size, and we will try to approximate the performance function based on the statistics from other papers\cite{ali2020batch,choi2021lazy,NVIDIA}.

The outcome of this work is a scheduling policy $\pi$. The average GPU throughput under policy $\pi$ is defined as:

\begin{equation}
\centering
    R^{avg}_{\pi} \triangleq \limsup\limits_{T\rightarrow\infty} \frac{1}{T} \sum_{t=1}^{T} R_{\pi}\left(b(t)\right).
\end{equation}

And our goal is to design a policy $\pi$ to maximize $R^{avg}_{\pi}$.
% \begin{equation}
% \centering
%     \max_{\{\mathbf{S}(1),\mathbf{S}(2),...\mathbf{S}(T)\}} R^{avg}
% \end{equation}
% \begin{equation}
% \centering
%     \max_{\pi} R^{avg}_{\pi}.
% \end{equation}


\section{Methodology}
By introducing another notation $G(t)$ to represent the remaining slots for the GPU to complete the current batch, we get the state $s(t) \triangleq \left(Q_{1}(t),Q_{2}(t),...Q_{N}(t), A_{1}(t),A_{2}(t),...A_{N}(t),G(t), b(t)\right) \in \mathcal{S}$, where $\mathcal{S}$ is the system state space. The action taken at slot $t$ is $a(t)\triangleq \mathbf{S}(t)$.

With the assumption that the distribution of $A_{i}(t)$ is time-invariant and service time is deterministic as a function of $b(t)$, we can formulate this problem as a \emph{constraint Markov decision progress} (CMDP), and the constraints are $\sum_{i=1}^{N} S_{i}(t)\leq B_{max}$, 
and $S_{i}(t)=0, \text{if } G(t)>1$. This can be solved by classic value iteration or policy iteration method.

Another solution is reinforcement learning, which is model-free and very popular nowadays. There are basic Q-Learning and other methods such as Actor-Critic that can help solve the problem.

==> Data/results_long.tex <==
\section{Numerical Results}\label{sec:results}
\begin{figure*}
\centering
\includegraphics[width=0.7\linewidth]{Figures/policy_view.eps}
\caption{The optimal policies for the average cost problem (\ref{eq7}) with energy and latency characteristics of GoogLeNet on TESLA P4.
The maximum batch size is chosen as $B_{\max}=32$.
The weights are
(a) $w_1 = 1, w_2 = 0.01$; (b) $w_1 = 1, w_2 = 0.1$; (c) $w_1 = 1, w_2 = 1$.} \label{policy_view}
\end{figure*}

\begin{figure}
\centering
\includegraphics[width=0.80\linewidth]{Figures/comparison.eps}
\caption{The comparison of different policies on the average cost, where $w_1=1$ and $w_2$ varies between $0$ and $20$.} \label{comparison}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=0.75\linewidth]{Figures/tradeoff.eps}
\caption{The time-energy tradeoff.} \label{tradeoff}
\end{figure}
% In this section, we demonstrate the numerical results of the optimal policy structures, the time-energy tradeoff and the performance comparison among different policies.
In this section, we take the GoogLeNet inference on TESLA P4 as the model, where the processing latency is $\tau^{[b]}=0.3051b+1.052$ (ms) and the energy consumption is ${\zeta}^{[b]}=19.90 b+19.60$ (mJ).
The maximum batch size $B_{max}$ is taken as 32.
% The long run average energy consumption will be exhibited with metric (mJ/ms), which is Watt (W).
The long run average energy consumption is measured by (mJ/ms), which is Watt (W).

Fig.~\ref{policy_view} demonstrates the policies obtained by solving the MDP under different $\rho$ and $w_2$.
Each row in the chart is a stationary deterministic policy, where each element denotes the action taken at the state corresponding to the column. 
% It can observed that the policies possess a control limit structure: The system should not serve until the state exceeds a threshold, which is called the \emph{control limit}. 
% This structure generally exists in the results of the experiments we have conducted, and thus we infer that it is a solid attribute of the optimal policies in our problem. 
It can concluded from the policies that the system should not serve until the state exceeds a threshold, which is called a \emph{control limit}.
This is exactly the conclusion in batch service queues with i.i.d. batch processing time\cite{deb1973optimal}.
% This conclusion generally exists in the experiments we have conducted, based on which we infer that the optimal policies of dynamic batching are in a control limit structure.
% The control limit structure generally exists in policies from numerous results, based on which we infer that it is a solid attribute of the optimal policies in our problem.
The control limit structure generally exists in policies from numerous results, and we believe it is an attribute that can be proved from theory.
From Fig.~\ref{policy_view}, we find that the control limit increases with $w_2$.
This is reasonable because the importance of energy consumption grows with $w_2$, and the energy is better saved with a larger batch size. 
Meanwhile, the control limit does not monotonically increase with $\rho$.
It is not surprising since the relationship between the response time and the control limit is not monotonic: A larger control limit introduces additional time of waiting to form a batch, but contributes to less average processing time and thus reduces the time of waiting for the end of former services.  
With an increasing $\rho$, the tradeoff between energy, response time and control limit is more complicated. 

We compare the SMDP solutions with the work-conserving policy and static batching policies with batch size $b=8,16,32$.
In the work-conserving policy, the server processes the maximum feasible batch of current requests and never waits for a new-coming request unless there is no waiting request.  
In static batching policies, the server always processes batches in a constant batch size, and waits for new-coming requests if there are not enough requests.
The static batching with $b=32$ is a special case called maximum batching policy in this setting where $B_{max}=32$.
It can be seen from Fig.~\ref{comparison} that the SMDP solution achieves the best among all policies under various parameter settings.
The work-conserving policy is far from optimal and the maximum batching policy works badly when $\rho=0.1$.
The other two static batching policies can approach the optimal policy under certain parameter scales.


The time-energy pairs reached with different $w_1,w_2$ are plotted in Fig.~\ref{tradeoff}.
By going through different $w_1,w_2$, the optimal policy of the weighted-objective SMDP can balance the response time and energy cost flexibly, where the pairs form a tradeoff curve given $\rho$ and the model of the server.
If there is any constraint on response time or power, we can find the optimal point on the curve and then search for the weight and policy corresponding to that point in a predefined chart.
The time-energy pairs of the work-conserving policy and maximum batching policy are the two end points of SMDP's tradeoff curve.
Meanwhile, the time-energy pairs of static batching policies do not necessarily lie on the curve.
A simple case is that static batching with $b=1$ is unstable when $\rho$ is large, leading to infinite average response time which is certainly not on the curve.
Nevertheless, some points of static batching policies are close to the tradeoff curve, which means that these policies can finely approximate the SMDP solution under certain parameters, and this agrees with the observation in Fig.~\ref{comparison}.



==> Data/solution_long.tex <==
\section{Procedure for Solving Infinite State SMDP}
% \subsection{Finite State Approximation to Infinite State Space}
% The procedure for solving the infinite state SMDP is composed of three stages: Firstly, a finite state SMDP is used to approximate the infinite state SMDP. Then, a discrete-time MDP is obtained by "discretizing" the finite state SMDP. At last, relative value iteration (RVI) is applied to the discrete-time MDP to solve the optimal policy.
% The stages are specified in the following subsections.
\subsection{Finite State Approximation}
% \subsection{State Space Truncation}
% Generalizing from the existence of a solution to the optimality equations in the discrete-time model, Theorem 11.4.6 \cite{puterman2014markov} gives the condition that an optimal stationary deterministic policy exists when the $\mathcal{S}$ is finite.
% However, it does not cope with our problem since we have $\mathcal{S}$ which is infinite but countable.
% It still needs some effort to dig out the condition in the countable state scenario.


The SMDP problem has infinite states in $\mathcal{S}=\{0,1,2,\ldots\}$, and is impractical to be solved by numerical methods.
% Hence, we introduce a \emph{finite} buffer with buffer size $s_{max}$ to approximate the infinite buffer.
% Hence, we truncate the infinite state space to a \emph{finite} state space $\mathcal{S}'=\{0,1,\ldots,s_{max},S_{o}\}$, by replacing the "tail" states which are larger than $s_{max}$ by an "overflow state" $S_{o}$.
Hence, we truncate the infinite state space to a \emph{finite} state space $\mathcal{S}'=\{0,1,\ldots,s_{max},S_{o}\}$, which replaces the states larger than $s_{max}$ by an "overflow" state $S_{o}$.
The dimension of the finite state space is $|\mathcal{S}'|=s_{max}+2$, where $s_{max}$ needs to be at least larger than $B_{max}$.
% To make the approximation accurate, $s_{max}$ needs to be large enough and at least greater than $B_{max}$.
% The truncated state space is $\mathcal{S}'=\{0,1,2,\ldots,s_{max},S_{o}\}$, $|\mathcal{S}'|=s_{max}+2$.
% The physical meaning of the state space truncation is to use a \emph{finite} buffer with size of $s_{max}$ to approximate the infinite buffer. And $S_{o}$ stands for the overflow case where at least one request is dropped since the buffer is full.
% The number of requests at the "overflow" state $S_{o}$ is also $s_{max}$, and original transitions to the "tail" states which are larger than $s_{max}$ are aggregated to $S_{o}$.
The rationale of the state space truncation is that the tail probability, the probability of being in the "tail" states $\mathcal{\hat{S}}=\{s_{max}+1,s_{max}+2,\ldots\}$, decreases with $s_{max}$.
When $s_{max}$ is large enough, the "tail" states are negligible.
Detailed analysis of convergence and error bounds of finite state approximation can be found in \cite{thomas1985finite}. 


% In the truncated model, the action space $\mathcal{A}$, the sojourn time distribution $f_{s,a}$, and the expected sojourn time $y(s,a)$ are the same as before, while the feasible action space at state $S_o$ is $A_{S_o}=\{0,1,2,...\min\{s_{max},B_{max}\}\}$.
In the truncated model, the action space $\mathcal{A}$, the sojourn time distribution $f_{s,a}$, and the expected sojourn time $y(s,a)$ are the same as before, while the feasible action space at state $S_o$ is $\mathcal{A}_{S_o}=\{0,1,\ldots,B_{max}\}=\mathcal{A}$ since $s_{max} > B_{max}$.
Original transitions to the "tail" states $\mathcal{\hat{S}}$ are aggregated to $S_{o}$, and
we assume the length of requests at $S_{o}$ is  $s_{max}$. 
The adapted transition probability $m'(j|s,a)$ for $\forall j,s \in \mathcal{S'}, \forall a \in \mathcal{A}_s$ is:
% The truncated state space is $\mathcal{S}'=\{0,1,2,\ldots,s_{max},S_{o}\}$, $|\mathcal{S}'|=s_{max}+2$, where $S_{o}$ stands for the overflow state where at least one request is dropped since the buffer is already full.
% (which should be adapted from small to large in the simulation, and stop when the output is stable),
% In the approximated model, the action space $\mathcal{A}$ and $\mathcal{A}_s$ keep the same, and so does $f_{s,a}$, while the adapted transition $m'(j|s,a)$ and cost $c'(s,a)$ are as follows:
\begin{equation}
\begin{aligned}
&m'(j|S_o,a) =\\
&\begin{cases}
p_{j-s_{max}+a}^{[a]}&  j \geq s_{max}-a, j \neq S_{o},a \neq 0\\
1-\sum\limits_{i=0}^{a}p_i^{[a]}
% =\sum\limits_{i=a+1}^{\infty}p_i^{[a]}
& j = S_{o},a \neq 0 \\
1& j=S_{o},a=0
\\
0& \text{ otherwise }
\end{cases},
\\
&m'(j|s,a) \; (s \neq S_o)=\\
&\begin{cases}
p_{j-s+a}^{[a]}& j \geq s-a, j \neq S_{o},a \neq 0 \\
1-\sum\limits_{i=0}^{s_{max}-s+a}p_i^{[a]}
% =\sum\limits_{i=s_{max}+1-s+a}^{\infty}p_i^{[a]}
&
j = S_{o},a \neq 0 \\
1& j = s+1,s<s_{max},a=0
\\
1& j=S_{o},s = s_{max},a=0
\\
0& \text{ otherwise }
\end{cases}.
\end{aligned}
\label{eqm}
\end{equation}

% \begin{equation}
% \begin{aligned}
% &m'(j|s,a) =\\
% &\begin{cases}
% p_{j-s+a}^{[a]}& \text{ $ j \geq s-a,$ $j \neq S_{o},$ $a \in \mathcal{A}_s,$ $a \neq 0$ } \\
% 1-\sum\limits_{i=0}^{s_{max}-s+a}p_i^{[a]}
% % =\sum\limits_{i=s_{max}+1-s+a}^{\infty}p_i^{[a]}
% &
% \text{ $ j = S_{o},$ $a \in \mathcal{A}_s,$ $a \neq 0$ } \\
% 1& \text{ $ j = s+1,$ $s<s_{max},$ $a=0$ }
% \\
% 1& \text{ $ j=S_{o},$ $s = S_{o}$ or $s_{max},$ $a=0$ }
% \\
% 0& \text{ otherwise }
% \end{cases}.
% \end{aligned}
% \label{eqm}
% \end{equation}

% \begin{equation}
% \begin{aligned}
% &c(s,a)= \\
% &\begin{cases}
%     w_2c^{[a]} +
%     w_1[s{\tau}^{[a]}+\frac{\lambda}{2}{({\tau}^{[a]})}^2]&  s \neq S_{o}, a \in \mathcal{A}_s, a \neq 0
%     \\
%     w_2c^{[a]} +
%     w_1[s_{max}{\tau}^{[a]}+\frac{\lambda}{2}{({\tau}^{[a]})}^2]&  s = S_{o}, a \in \mathcal{A}_s, a \neq 0
%     \\
%     w_1s/{\lambda}&  s \leq s_{max}, a = 0
%     \\
%     % c(s,0) =& \; overflow \; cost, \quad s=S_{o}
%     w_1s_{max}/{\lambda}&  s=S_{o}, a = 0
% \end{cases}.
% \end{aligned}
% \end{equation}
% \begin{equation}
% \begin{aligned}
% &c(s,a)= \\
% &\begin{cases}
%     w_2c^{[a]} +
%     w_1[s{\tau}^{[a]}+\frac{\lambda}{2}{({\tau}^{[a]})}^2]&  s \neq S_{o}
%     \\
%     w_2c^{[a]} +
%     w_1[s_{max}{\tau}^{[a]}+\frac{\lambda}{2}{({\tau}^{[a]})}^2]&  s = S_{o}
%     \\
% \end{cases},\\
% &a \in \mathcal{A}_s, a \neq 0,
% \end{aligned}
% \end{equation}

% \begin{equation}
% \begin{aligned}
% &c(s,0)= \\
% &\begin{cases}
%     w_1s/{\lambda}&  s \leq s_{max}
%     \\
%     % c(s,0) =& \; overflow \; cost, \quad s=S_{o}
%     w_1s_{max}/{\lambda}&  s=S_{o}
% \end{cases}.
% \end{aligned}
% \end{equation}

% \begin{equation}
% \begin{aligned}
% &c(s,a)= \\
% &\begin{cases}
%     w_2c^{[a]} +
%     w_1[s{\tau}^{[a]}+\frac{\lambda}{2}{({\tau}^{[a]})}^2]&  s \neq S_{o}, a \in \mathcal{A}_s, a \neq 0
%     \\
%     % w_2c^{[a]} +
%     % w_1[s_{max}{\tau}^{[a]}+\frac{\lambda}{2}{({\tau}^{[a]})}^2]&  s = S_{o}, a \in \mathcal{A}_s, a \neq 0
%     % \\
%     w_1s/{\lambda}&  s \neq S_{o}, a = 0
%     \\
%     % c(s,0) =& \; overflow \; cost, \quad s=S_{o}
%     % w_1s_{max}/{\lambda}&  s=S_{o}, a = 0
% \end{cases},
% \end{aligned}
% \end{equation}
% \begin{equation}

% \end{equation}

% \begin{equation}
% \begin{aligned}
% &c'(s,a)= c(s,a), \quad s \neq S_o,\\
% &c'(S_{o},a)= \\
% &\begin{cases}
%     % w_2c^{[a]} +
%     % w_1[s{\tau}^{[a]}+\frac{\lambda}{2}{({\tau}^{[a]})}^2]&  s \neq S_{o}, a \in \mathcal{A}_s, a \neq 0
%     % \\
%     w_2c^{[a]} +
%     w_1[s_{max}{\tau}^{[a]}+\frac{\lambda}{2}{({\tau}^{[a]})}^2]&  a \in \mathcal{A}_s, a \neq 0
%     \\
%     % w_1s/{\lambda}&  s \leq s_{max}, a = 0
%     % \\
%     % c(s,0) =& \; overflow \; cost, \quad s=S_{o}
%     w_1s_{max}/{\lambda}&  a = 0
% \end{cases}.
% \end{aligned}
% \end{equation}
% In the primal problem, the infinite state space leads to unbounded holding cost, which is also erased by the truncation.
The unbounded holding cost induced by the infinite states in the primal problem is also erased by the truncation.
% Therefore, we introduce an additional cost $c_oy(s,a) \; (c_o \geq 0)$ into the cost at the "overflow" state $S_o$, working as an estimation of the difference between the expected holding cost at "tail" states and the holding cost at $s_{max}$.
Therefore, we introduce an additional cost $c_oy(s,a) \; (c_o \geq 0)$ to the "overflow" state $S_o$, working as an estimation of the difference between the expected holding cost at "tail" states and the holding cost at $s_{max}$.
The adapted cost $c'(s,a)$ is:
% $C_o$ works as an estimation of the average number of the "tail" states
% which have the same feasible action space, $y(s,a)$ is 
% as a replacement for the expected holding cost (which is the main part of the total cost) in the erased long tail states:
\begin{equation}
\begin{aligned}
c'(s,a)= 
\begin{cases}
    c(s_{max},a)+c_oy(s,a) \quad s = S_o \\
    c(s,a) \quad \quad \quad \quad \; s \neq S_o, s \in \mathcal{S'}
\end{cases},
\end{aligned}
\forall a \in \mathcal{A}_s.
\label{eq13}
\end{equation}
Since $\rho \in [0,1)$, the optimal policy must stabilize the system.
The additional cost can be also interpreted as an overflow punishment, which pushes the optimal policy away from causing overflow.
% Note that for the "tail" states, holding cost is increasing and will become the main part of the total cost.
% The dimension of the state space heavily impacts the computation complexity of algorithms, and therefore it is appreciated to further reduce $|\mathcal{S}'|$.
% It is appreciated to further reduce the length of the truncated state space $|\mathcal{S}'|$, so as to decrease the computation complexity of algorithms.
% To reach this end, we introduce an additional cost $c_o'(j |s,s)$ to punish the transition to the state $S_o$:
% To reach this end, we introduce an additional cost $c_o(j |s,s)$ to punish the transition to the 
% In our problem, the infinite state space also leads to unbounded holding cost.
% Therefore, we introduce an additional cost $c_o'(j |s,s)$ as a replacement for the holding cost (which is the main part of the total cost) in the erased long tail states:
% \begin{equation}
%     c_o'(j|s,a)=
%     \begin{cases}
%     C_o y(s,a) & \quad j=S_o
%     \\
%     0&
%     \quad \text{otherwise}
%     \end{cases},
% \end{equation}
% where $C_o$ is a constant, which can also be interpreted as the overflow punishment.
% The rationale is that $c_o'(j|s,a)$ works as a replacement for the holding cost (which is the main part of the total cost) in the erased long tail states
Note that the additional cost in (\ref{eq13}) is scarcely mentioned in the literature, without which the problem can be solved as well but with a larger satisfactory $s_{max}$ and more computation rounds in value-based iteration algorithms.
% Meanwhile, the additional cost should not be too large.

We establish a criterion to assess the approximation regarding the difference in average cost: Given a stationary deterministic policy as a function $\pi:\mathcal{S'} \rightarrow \mathcal{A}$, the corresponding state transition matrix is $P_{{\pi}} \in \mathbb{R}^{{|\mathcal{S'}|}\times{|\mathcal{S'}|}}$.
Suppose that the Markov chain with $P_{\pi}$ has a unique stationary distribution $\bm{\mu}=(\mu_0,\mu_1,\ldots,\mu_{S_o})$.
Then the average cost per unit time is:
\begin{equation}
    g^{\pi}= \frac{\sum_{s \in \mathcal{S'}} \mu_s \cdot c(s,\pi(s))}{\sum_{s \in \mathcal{S'}} \mu_s \cdot y(s,\pi(s)) }.
\end{equation}
Let $\Delta^{\pi}$ be the average cost contributed by $S_o$ per unit time:
\begin{equation}
    \Delta^{\pi}= \frac{\mu_{S_o} \cdot c(S_o,\pi(S_o))}{\sum_{s \in \mathcal{S'}} \mu_s \cdot y(s,\pi(s)) }.
\end{equation}
Given a predefined constant $\delta>0$, if $\Delta^{\pi} < \delta$, we state that the approximation is acceptable with tolerance $\delta$.
If not, a larger $s_{max}$ should be selected.
% which is expected to be zero in an ideal approximation
 
The optimality equations of the finite state SMDP are:
% \begin{equation}
% \begin{aligned}
% h(s)=\min _{a \in {\mathcal{A}}_s}\Bigg\{ 
% &c'(s,a)-gy(s,a)  \\
% +&\sum_{j \in S} {m'}(j|s, a) \left[c_o'(j|s,a)+h(j)\right]\Bigg\}.
% \end{aligned}
% \end{equation}
\begin{equation}
\begin{aligned}
h(s)=\min _{a \in A_s}\Bigg\{c'(s, a)-g y(s, a)+\sum_{j \in S'} m'(j | s, a) h(j)\Bigg\},
\end{aligned}
\label{optimality3}
\end{equation}
for $\forall s \in \mathcal{S'}$.
Denote $g^*$ as the optimal average expected cost in the finite state SMDP.

\begin{figure*}
\centering
\includegraphics[width=0.7\linewidth]{Figures/policy_view.eps}
\caption{The optimal policies for the average cost problem (\ref{eq7}) with energy and latency characteristics of GoogLeNet on TESLA P4.
The maximum batch size is chosen as $B_{max}=32$.
The weights are
(a) $w_1 = 1, w_2 = 0.01$; (b) $w_1 = 1, w_2 = 0.1$; (c) $w_1 = 1, w_2 = 1$.} \label{policy_view}
\end{figure*}

\subsection{Associated Discrete-Time MDP}
The finite state continuous-time SMDP is associated with a \emph{discrete-time} MDP through a "discritization" transformation (See Chapter 11.4 in \cite{puterman2014markov}).
% Since this is a countable-state model,  it can be transformed to a discrete-time model and the existence of a solution to the optimality equation, can be established.  
% Denote all quantities in the transformed model with “$\sim$”. Let $\tilde{\mathcal{S'}}=\mathcal{S'}$, $\tilde{\mathcal{A}_s}=\mathcal{A}_s$ for all $s \in \mathcal{S}$, 
The state space $\mathcal{S'}$, the action space $\mathcal{A}$ and the feasible action space $\mathcal{A}_s$ for any $s \in \mathcal{S'}$ keep unchanged in the transformed model.
The transformed cost $\tilde{c}(s, a)$ and the transformed transition probability $\tilde{m}(j | s, a)$ for $\forall j,s \in \mathcal{S'}, \forall a \in \mathcal{A}_s$ are
\begin{equation}
\begin{aligned}
    \tilde{c}(s, a) \triangleq& \; c'(s, a) / y(s, a),\\
    \tilde{m}(j | s, a) \triangleq& 
    \begin{cases}
    \eta m'(j | s, a) / y(s, a)& j \neq s \\ 
    1+\eta[m'(s| s, a)-1] / y(s, a)& j=s
    \end{cases},
\end{aligned}
\end{equation}
where $\eta$ satisfies
\begin{equation}
    0<\eta<y(s, a)/(1-m'(s|s, a)),
\end{equation}
for all $a \in A_s$ and $s \in S'$ for which $m'(s|s, a)<1$. 

% To find a parameter $\eta$ for the transformation, we have to calculate the lower bound of $\frac{y(s,a)}{1-m'(s|s,a)}$:
By (\ref{eqy}) and (\ref{eqm}), for $\forall s \in {\mathcal{S}'}, \forall a \in {\mathcal{A}_s} \text{ s.t. } m'(s|s, a)<1$, we have
\begin{equation}
\begin{aligned}
    \frac{y(s,a)}{1-m'(s|s,a)}=
    \begin{cases}
        1/\lambda& a=0, s \neq S_o
        \\
        {\tau}^{[a]}/(1-p_a^{[a]})& a \neq 0, a \in {\mathcal{A}}_s, s \neq S_o
        \\
        {\tau}^{[a]}/\sum\limits_{i=0}^{a}p_i^{[a]}& a \neq 0, a \in {\mathcal{A}}_s, s = S_o
    \end{cases},
\end{aligned}
\end{equation}
% Therefore, we have to choose one $\eta$ that satisfies $0<\eta<\min\{\frac{1}{\lambda},\min_{a \in \mathcal{A}}\{\frac{{\tau}^{[a]}}{1-p_a^{[a]}}\}\}$.
Therefore, an appropriate $\eta$ should satisfy
\begin{equation}
  0<\eta<\min\Bigg\{\frac{1}{\lambda},\min_{a \in \mathcal{A}}\bigg\{
  \frac{{\tau}^{[a]}}{1-p_a^{[a]}}, \frac{{\tau}^{[a]}}{\sum\limits_{i=0}^{a}p_i^{[a]}}
  \bigg\}\Bigg\}.  
\end{equation}
And we find from experiments that the larger the $\eta$ is, the faster the value-based iteration algorithm converges.

% Further, let $\tilde{g}^\pi$ denote the average expected reward for policy $\pi$ and $\tilde{g}^*$ denote the optimal gain for the transformed model.
For the discrete-time MDP, the optimality equations are
% \begin{equation}
% h=\min _{d \in D^{\mathrm{MD}}}\left\{\tilde{c}_d-g e+\tilde{M}_d h\right\},
% \label{eq11}
% \end{equation}
% or written in
\begin{equation}
h(s)=\min _{a \in {\mathcal{A}}_s}\Bigg\{\tilde{c}(s,a)-g +\sum_{j \in S'} \tilde{m}(j|s, a) h(j)\Bigg\},
\forall s \in \mathcal{S'}.
\label{eq12}
\end{equation}
% for $\forall s \in \mathcal{S'}$.
% \begin{equation}
% h(s)=\min _{a \in {\mathcal{A}}_s}\left\{\tilde{c}(s,a)-g +\sum_{j \in S} \tilde{m}(j|s, a) \left(c'(j|s,a)+h(j)\right)\right\}.
% \end{equation}
By Proposition 11.4.5 in \cite{puterman2014markov}, if $(\tilde{g},\tilde{h})$ satisfy the discrete-time optimality equations in (\ref{eq12}), then $(\tilde{g},\eta\tilde{h})$ satisfy (\ref{optimality3}) and $\tilde{g}=g^*$ is the optimal average cost in the continuous-time model.
% The optimal policy obtained by solv the discrete-time MDP is also optimal in the continuous-time SMDP.
And Theorem 11.4.6 in \cite{puterman2014markov} clarifies the existence of an average optimal stationary deterministic policy. 



% We then apply the discrete transformation to the continuous model and get the corresponding $\tilde{c},\tilde{m}$.


% Then the optimality function of the transformed model is:

% \begin{equation}
% h(s)=\min _{a \in {\mathcal{A}}_s}\left\{\tilde{c}(s,a)-g +\sum_{j \in S} \tilde{m}(j|s, a) h(j)\right\}.
% \end{equation}

% And later, we use the relative value iteration algorithm to solve the discrete MDP problem.
% Although it is argued in other papers that the RVI can be directly applied in the continuous setting, we do not believe it's true for the infinite space case, since the overflow punishment would interact with the state sojourn time, which is hard to be added in the original formula since the average cost is calculated by summing up infinite terms.

\subsection{Relative Value Iteration}
In this paper, we utilize value-based iteration algorithms to solve the discrete-time MDP.
Specifically, in the average cost MDP, the standard value iteration is numerically unstable, so we use relative value iteration (RVI)\cite{puterman2014markov} instead.

Let $J_{n}(s)$ be the value function at state $s \in \mathcal{S'}$ in the $n$th epoch, where $n \in \mathbb{N}$.
At the beginning of the algorithm, a state $s^* \in \mathcal{S'}$ is arbitrarily chosen.
The iterative formula of RVI is 
\begin{equation}
    J_{n+1} (s)=\min _{a \in A_s}\Bigg\{\tilde{c}(s, a)-J_{n} (s^*)+\sum_{j \in S'} \tilde{m}(j | s, a) J_{n}(j)\Bigg\}.
\end{equation}
The key point is that in each iteration, the value function of $s^*$ is subtracted from the standard Bellman equation.
$J_{n} (s)$ finally converges to the relative value function at $s$.
% The function $J_n(s)$ will finally converge to the relative value function $h(s)=v(s)-g$.

% \begin{algorithm}
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
% \caption{Relative Value Iteration Algorithm} 
% 	\begin{algorithmic}[1]
%     	\REQUIRE {$S',\tilde{c}(s,a),\tilde{m}(j|s,a)$;}
% 	    \ENSURE {${\pi}^{*}$;}
% 	    \STATE {Initialize $J_0(s)=0$ for all $s \in \mathcal{S'}$;}
% 	    \STATE {Select a state $s^{*}$;}
% 	    \FOR {$n:=1$ to $\infty$}
% 	    \FOR {each $s \in \mathcal{S'}$}
% 	    \STATE {Compute $J_{n+1} (s)=\min _{a \in A_s}\Bigg\{\tilde{c}(s, a)-J_{n} (s^*)+\sum_{j \in S'} \tilde{m}(j | s, a) J_{n}(j)\Bigg\}$;}
% 	   % \STATE {Compute $J_{n+1} (s) = R_{n+1} (s)-R_{n+1} (s^*)$}
% 	    \ENDFOR
% 	    \IF {$sp(J_{n+1}-J_n)<\epsilon $}
% 	    \STATE {break;}
% 	    \ENDIF
% 	    \ENDFOR
% 	    \FOR {each $s \in \mathcal{S'}$}
% 	    \STATE {$a^{*}_s \in \arg \min_{a \in A_s} \Bigg\{\tilde{c}(s, a)-J_{n} (s^*)+\sum_{j \in S'} \tilde{m}(j | s, a) J_{n}(j)\Bigg\}$;}
% 	    \ENDFOR
% 	    \STATE {
% 	    ${\pi}^{*} = (a^{*}_1, a^{*}_2, \dots , a^{*}_{S_o})$;
% 	    }
%     \end{algorithmic}
% \end{algorithm}
The number of multiplications per iteration in RVI is $\sum \limits_{s \in \mathcal{S'}} |\mathcal{A}_s||\mathcal{S'}| \approx B_{max}s_{max}^2$.

As aforementioned, the optimal policy of the discrete-time MDP is also optimal in its associated finite state SMDP.
Furthermore, it should be optimal in the original infinite state SMDP as well if the finite state approximation is accurate enough.

==> Data/system_model.tex <==
\section{System Model}\label{sec:system}
\subsection{Poisson Arrival}
Suppose that the arrival of inference tasks follows Poisson Process.
Since the tasks from different users are of the same model and are indifferent for the GPU server, we consider the total arrival of users.
The total arrival rate is denoted as $\lambda$.
The number of task arrivals in a period of $t$ follows Poisson distribution with parameter $\lambda t$.

\subsection{Deterministic and Batch-Dependent Service Time}
According to Section~\ref{sec:GPU}, the service time of GPU is deterministic and the exact value is a linear function of batch size.
Let $b$ denote the batch size, $b \in \{1,2,3,\dots,B_{\max}\}$, where $B_{\max}$ is the maximum number of batch size.
Then the batch processing latency is $L(b)=Ab+C$.
Given the GPU and inference model, the parameters $B_{max}$, $A$ and $C$ are determined.
% In our experiment setting shown in Fig.~\ref{fig:fitting}, the $B_{max}$ is 36 and $L(b)=7.8699b+38.1243 (ms)$.

Let $Th(b)$ denote the GPU throughput, then $Th(b)=b/L(b)=b/(Ab+C)$.
Since the throughput is monotonically increasing regarding b, the maximum service rate ${\mu}_{max}=Th(B_{max})$.
Suppose $\lambda < {\mu}_{max}$, which is the stability condition.

\subsection{Energy Consumption}
Similar to latency, the energy consumption of a batch process is $E(b)=\bar{A}b+\bar{C}$.
The energy efficiency $Ee(b)$ is defined as the average number of tasks served with one unit of energy consumption: $Ee(b)=b / (\bar{A}b+\bar{C})$.
The larger the batch size is, the higher the energy efficiency is.

\subsection{Buffer}
Since we only consider the total arrival, the system is a single queue system with only one buffer.
The tasks waiting to be processed are stored in the buffer.
The queue length in the buffer is represented by $s$, and $s \in \{0,1,2,\dots,BF_{max}\}$.
The $BF_{max}$ stands for the maximum buffer size, which can be infinitely large.

\subsection{M/G/1 Queuing System under Stationary Markovian Policy}
In addition to assumptions of Poisson arrival and deterministic and batch-dependent service time, we suppose the system is working under a stationary Markovian policy.
Then the system is a M/"D"/1 queuing system, where the "D" stresses the difference between the batch-dependent service time and ordinary deterministic distribution.
This queuing system does not possess Markov property because of non-exponential service time.

Using the method of imbedded Markov chain, if we focus on the queuing state only at action points, the system is then a Continuous Time Markov Chain (CTMC).

\subsection{Objective Functions}
% We aim to find the optimal stationary Markovian policy, which is only 
In queuing systems, the long time average objective is suitable to be considered.
Specifically, there are different objectives according to different requirements.
In the following statements, we use $\pi$ to denote the policy.
\begin{itemize}
    \item \emph{minimize (task) average waiting time / minimize (time) average queue length}: 
    
    This objective aims to optimize the service quality, that is to say to minimize the average waiting time of a task. Since it is not easy to directly optimize the waiting time, which needs a large amount of delay observations, we turn to minimize the average queue length $s^{avg}_{\pi}$:
    \begin{equation}
    \centering
    s^{avg}_{\pi} \triangleq \limsup\limits_{T\rightarrow\infty} \frac{1}{T} \sum_{t=1}^{T} s_{\pi}\left(t\right).
    \end{equation}
    By Little's Law, it is equivalent to minimize the average waiting time $t^{avg}_{\pi}$: 
    \begin{equation}
    \centering
    t^{avg}_{\pi} \triangleq
    \frac{1}{\lambda}{s^{avg}_{\pi}}
    =
    \limsup\limits_{T\rightarrow\infty} \frac{1}{\lambda T} \sum_{t=1}^{T} s_{\pi}\left(t\right).
    \end{equation}
    
    \item \emph{maximize (time) average throughput}: 
    
    This objective is optimized from the perspective of the GPU server.
    If we suppose the cost of running a GPU server is almost the same as long as the server is on, then it's natural to make the server process as many jobs as possible, which is to maximize the long time average throughput ${Th}^{avg}_{\pi}$:
    \begin{equation}
    \begin{aligned}
    \centering
    {Th}^{avg}_{\pi} 
    &\triangleq \limsup\limits_{T\rightarrow\infty} \frac{1}{T} \sum_{t=1}^{T} {Th}\left(b_{\pi}(t)\right)
    &=
    \limsup\limits_{T\rightarrow\infty} \frac{1}{T} \sum_{i=1}^{N(T)} {Th}\left(b_{\pi}^i\right)*D(b_{\pi}^i)
    &=
    \limsup\limits_{T\rightarrow\infty} \frac{1}{T} \sum_{i=1}^{N(T)} b_{\pi}^i
    .
    \end{aligned}
    \end{equation}
    The $i$ stands for the $i$th batch processing and $N(T)$ is the last batch processing before time $T$.
    
    Now we discover that it is \emph{meaningless} to maximize it in our setting since the average throughput is equal to the arrival rate $\lambda$ in stable state.
    
    \item \emph{minimize (task) average latency/ maximize computational efficiency}: 
    
    This objective is also based on the server.
    The average latency is different from aforementioned average waiting time.
    The average latency is the average computation time in the GPU, while the average waiting time is the average queuing time in the buffer.The average latency is ${D}^{avg}_{\pi}$:
    
    \begin{equation}
    \centering
    D^{avg}_{\pi} 
    \approx
    \limsup\limits_{T\rightarrow\infty} \frac{1}{\lambda T} \sum_{i=1}^{N(T)} D\left(b_{\pi}^i\right).
    \end{equation}
    The computational efficiency is ${Ce}^{avg}_{\pi}$:
    \begin{equation}
    \begin{aligned}
    \centering
    {Ce}^{avg}_{\pi} 
    &\triangleq
    \limsup\limits_{T\rightarrow\infty} \frac{\sum_{i=1}^{N(T)} b_{\pi}^i}
    {\sum_{i=1}^{N(T)} D\left(b_{\pi}^i\right)}
    &\approx
    \limsup\limits_{T\rightarrow\infty} \frac{\lambda T} {\sum_{i=1}^{N(T)} D\left(b_{\pi}^i\right)}
    =
    \frac{1}{D^{avg}_{\pi}}
    .
    \end{aligned}
    \end{equation}
    Hence, maximizing ${Ce}^{avg}_{\pi}$ is equivalent to minimizing $D^{avg}_{\pi}$.
    
    \item \emph{minimize (task) average energy consumption/ maximize energy efficiency}:
    
    Similarly, we have average energy consumption $E^{avg}_{\pi}$ and average energy efficiency $Ee^{avg}_{\pi}$:
    \begin{equation}
    \centering
    E^{avg}_{\pi} 
    \approx
    \limsup\limits_{T\rightarrow\infty} \frac{1}{\lambda T} \sum_{i=1}^{N(T)} E\left(b_{\pi}^i\right),
    \quad
    {Ee}^{avg}_{\pi}= \frac{1}{E^{avg}_{\pi}}.
    \end{equation}
    The energy efficiency is more \emph{meaningful} than computational efficiency, because it reduces the carbon emission and reduce the considerable cost on energy, e.g. electric power.
    
    \item \emph{minimize weighted average queue length and average energy consumption}:
    
    A rational objective is considered both from the user's perspective and the server's perspective.
    Suppose we aim to minimize $w1*t^{avg}_{\pi} + w2*E^{avg}_{\pi}$, where $w1$ and $w2$ are weights that are no less than zero.
    % Then our objective becomes:
    % \begin{equation}
    %     \min \quad \limsup\limits_{T\rightarrow\infty} \frac{1}{\lambda T}
    %     \left(
    %     w1*\sum_{i=1}^{N(T)} s_{\pi}^i
    %     +
    %     w2*\sum_{i=1}^{N(T)} E\left(b_{\pi}^i\right)
    %     \right)
    %     ,
    % \end{equation}
    Then our objective becomes:
    \begin{equation}
        \min \quad \limsup\limits_{T\rightarrow\infty} \frac{1}{\lambda T}
        \left(
        w1*\sum_{i=1}^{T} s_{\pi}(t)
        +
        w2*\sum_{i=1}^{N(T)} E\left(b_{\pi}^i\right)
        \right)
        ,
    \end{equation}
    % which is equivalent to
    % \begin{equation}
    %     \min \quad \limsup\limits_{T\rightarrow\infty} \frac{1}{\lambda T}
    %     \sum_{i=1}^{N(T)}
    %     \left(
    %     w1* s_{\pi}^i
    %     +
    %     w2*E\left(b_{\pi}^i\right)
    %     \right)
    %     ,
    %     \label{objective}
    % \end{equation}
    which is equivalent to
    \begin{equation}
        \min \quad \limsup\limits_{T\rightarrow\infty} \frac{1}{\lambda T}
        \sum_{i=1}^{T}
        \left(
        w1* s_{\pi}(t)
        +
        w2*E\left(b_{\pi}(t)\right)
        \right)
        ,
        \label{objective}
    \end{equation}
    or
    \begin{equation}
        \min \quad \limsup\limits_{T\rightarrow\infty} \frac{1}{T}
        \sum_{t=1}^{T}
        \left(
        w1* s_{\pi}(t)
        +
        w2* e_{\pi}(t)
        \right)
        ,
    \end{equation}
    where $e_{\pi}(t)$ is the power consumption equal to $E\left(b_{\pi}^i\right)$ averaging on the total batch processing time.
    Then the goal is to minimize the weighted average queue length and average energy consumption.
\end{itemize}
